Tweeting MPs: Digital Engagement between Citizens and Members of Parliament in the UK

Disengagement and disenchantment with the Parliamentary process is an important concern in today's Western democracies. Members of Parliament (MPs) in the UK are therefore seeking new ways to engage with citizens, including being on digital platforms such as Twitter. In recent years, nearly all (579 out of 650) MPs have created Twitter accounts, and have amassed huge followings comparable to a sizable fraction of the country's population. This paper seeks to shed light on this phenomenon by examining the volume and nature of the interaction between MPs and citizens. We find that although there is an information overload on MPs, attention on individual MPs is focused during small time windows when something topical may be happening relating to them. MPs manage their interaction strategically, replying selectively to UK-based citizens and thereby serving in their role as elected representatives, and using retweets to spread their party's message. Most promisingly, we find that Twitter opens up new avenues with substantial volumes of cross-party interaction, between MPs of one party and citizens who support (follow) MPs of other parties.

==> sections/caseStudies.tex <==
\section{Case Studies (1.5 pages)}\label{sec:caseStudies}

\paragraph{Case Study}
 \#Brexit (108 days), \\
 \#WestminsterScandal 10 days.

\subsection{Brexit engagements and several uprisings}
Data - 5 Sept to 21 Dec (both included, 108 days), i.e starting after first summer recess return of the House till Christmas recess on 21 Dec 2017. \url{http://www.parliament.uk/about/faqs/house-of-commons-faqs/business-faq-page/recess-dates/}. Moreover, data is from post 2017 General Elections where conservative lost their parliamentary majority. This maintains the uniformity of same MPs (post 2017 elections) track down in the data. Intuitively true that for out of the context data of 25 Dec, it recorded the least posts in last six months. Hence, Christmas does not deal with with politics and is celebrated by all, above the common difference in House of Commons.
Used Streaming API to fetch UK (225 m),EU (53.22 lat, 6.06long,1300 mile) and across the globe activity for ``\#Brexit''. This is done using scheduled task in R, \ie automatically. Daily two times running the script file on HPC generates data and dump csv. Files missing from last eight days checked and generated. This ensure that data is fetched if script fails for one of two times in a day or in subsequent days. API limit historical data to roughly 10 days hence this approach carve out the problem and create data for use.
\begin{center}
	\begin{tabular}{ |c|c|c| } 
		\hline
		UK Tweeet & EU-UK Tweet & Global-EU*s \\ 
		\hline
		573739    & 670738      & 1146749\^{}   \\ 
		\hline
	\end{tabular}
\end{center}

*UK is still a part of EU.
\^Although take care but Global-EU may have some UK and EU activity. IF a user neither gave a geo-code with a tweet nor his/her profile location matches a places near by or inside UK then the tweet will be recorded as global. Twitter API or specifically Twitter records location by place ID when annotated with place else roll back to a user’s profile location and geo-code the user. Say London or UK would \pa{comes for geo-code, radius} However a user is free to give any option of his/her choice. The examples exist here are text field like- worldwide, earth, etc. Nevertheless, UK and EU-UK geotagged data is of high confidence.

Why Brexit is know as Brexit?
Popular events in data
Mentions and MPs activity in this
Westminster scandal
Figures

\subsection{Westminster Scandal created a witch hunt}
\ew{Timeline- To be mailed.
Count of MPs who resigned \eg{Damian Green, Michel Fallen}.
There are four possible outcomes when an MPs is affected by scandal. They may resign or be sacked from ministerial or other roles and they may resign or be recalled (sacked) as an MP. Social media and main stream media are both likely to be influential in this process and negative comment in one is likely to reinforce negative comment and the other. However, they overall political impact on the government or party is likely to be a complex calculation. If the negative comment is likely to die down quickly the MP or the Prime minister may conclude that the least negative outcome for the party is for the MP to remain in post, at least for the time being.
}

Volume of Tweets, split across party and gender and age.
Whether in support or criticism of the issue.
General tone - negative or positive (compare with general \#MeToo for Westminster scandal, and with journalists tone on Brexit for Brexit.)

\subsection{Twitter for Poll. What legislation to Propose?}
\begin{figure}
	\centering
	\includegraphics[width=\columnwidth]{figs/ChrisBryantSurvey}
	\caption{ChrisBryant Survey and mentions to him}
	\label{fig:ChrisBryantSurvey}
\end{figure}
\ew{Timeline of bill becoming an act, beck bench MP.
Four reasons of having a poll of private members bills-\\
1) Publicity for the MP. \\
2) Publicity for the bill. The more publicity a bill receives the more likely it is to become law.\\
3) MP think that getting ideas from the public will lead to better legislation. 
4) MP thinks that the public should participate in the legislative process which is know as Direct Democracy.
This case may contains portions of each of these bits. }

\ew{example of a non-Government backbench MP (Chris Bryant) using a Twitter poll to decide what legislation to propose.
\url{https://twitter.com/RhonddaBryant/status/885111797874925568/photo/1?ref_src=twsrc\%5Etfw\&ref\_url=https\%3A\%2F\%2Fd-0170667487247821430.ampproject.net\%2F1513979839742\%2Fframe.html}
Information about his Private Member’s Bill is here:
\url{https://services.parliament.uk/bills/2017-19/assaultsonemergencyworkersoffences.html}
He succeeded in getting support from the Government, which means that the Bill is very likely to become law:
\url{http://www.huffingtonpost.co.uk/entry/assaults-on-emergency-workers-bill-set-for-government-backing-chris-bryant_uk_59e3c3f4e4b03a7be5816c51}}




%The previous section has highlighted the nature of social broadcast, focussing on the large number of unwatched and unpopular streams. Next, we inspect the opposite end of the spectrum --- highly popular streams. A unique aspect of Facebook Live is that it provides the locations of stream viewers for broadcasts with an audience of 100+. This allows us to understand the geographical relationship between broadcasters and viewers.
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Where are the users?} \label{sec:geo:where}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%We begin by  inspecting the locations of users to understand where Facebook Live's userbase is. Figure~\ref{fig:bcast_view_map} presents viewer (blue) and broadcaster (green) locations for any streams that garner above 100 viewers. This covers 45K broadcasts, and 20.3 million viewers. The map shows a significant spread of broadcasters (green) with a focus on East Coast US, Brazil, Europe and South East Asia. It can be seen that most major conurbations are covered. A particularly nice feature of the dataset is that locations are based on mobile GPS-based geo-tags (rather than IP address). This gives us accurate geographical vantage into regions such as China, which typically access Facebook via VPN (thereby changing their reported IP geolocation). It can be seen that despite the blocking of Facebook, there are a number of users in China. In the rest of this section, we focus on the top 19 countries measured by broadcasters and consumers. These countries are obtained taking the union of the top 15 countries in terms of broadcasters and top 15 in terms of consumers. 
%
%Figure~\ref{fig:bcaster_vs_viewer} presents the percentage of broadcasters and viewers based in each of the top 19 countries. A clear ranking can be observed; the US dominates both the number of broadcasters and viewers, followed by Thailand and Vietnam. The latter is particularly interesting, as in many cases we find that the number of viewers and broadcasters in a country do not necessarily correlate. For instance, whereas, in the US or Brazil, the fraction of viewers and broadcasters is relatively \emph{similar}, Thailand generates a significant proportion of the world's broadcasts (11.26\%), but only constitutes 8\% of the viewers. Conversely, in Turkey, there are significant fraction of viewers (7.1\% of the world's viewers), but only 2.94\% of broadcasters. Similar observations can be made across many other countries, including Korea, Peru and Romania. Through manual inspection, we find a number of potential reasons. For instance, Turkey blocks access to Facebook; therefore, most users are likely accessing it via circumvention tools. Whereas Turkish users may be keen on consuming content, they may be less willing to expose themselves by broadcasting on a censored medium. In the case of Thailand, we find that a notable portion of adult content is being streamed, and this niche content attracts a globally distributed viewership (rather than just in Thailand). 
%
%
%%\begin{figure}[ht]
%%%\vspace{-1.5em}
%% \centering
%%\includegraphics[width=0.95\linewidth]{figs/v2/broadcasters_viewers.png}
%%% \subfloat{\includegraphics[height=0.4in]{figs/cmap}} 
%%%\vspace{-1.5em}
%%\caption{Locations of broadcasters and viewers across the globe}
%%\label{fig:bcast_view_map}
%%\end{figure}
%
%
%\begin{figure}[t]
%	%\vspace{-1.5em}
%	\centering
%	\includegraphics[width=1.0\linewidth]{figs/v3/world_map.png}
%	% \subfloat{\includegraphics[height=0.4in]{figs/cmap}} 
%	%\vspace{-1.5em}
%	\caption{Locations of influential broadcasters ($>$100 viewers) and the respective viewers across the globe}
%	\label{fig:bcast_view_map}
%\end{figure}
%
%
%
%\begin{figure}[h]
%	%\vspace{-1.5em}
%	\centering
%	\includegraphics[width=0.95\linewidth]{figs/v3/bcaster_vs_viewer}
%	\caption{Broadcasters and viewers across top-accessed  countries.}
%	\label{fig:bcaster_vs_viewer}
%\end{figure}
%
%
%
%
%
%%\begin{figure}[ht]
%%%\vspace{-1.5em}
%% \centering
%%\includegraphics[width=0.95\linewidth]{figs/v2/user_gen_vid_distrib_4_sample}
%%% \subfloat{\includegraphics[height=0.4in]{figs/cmap}} 
%%%\vspace{-1.5em}
%%\caption{\% of broadcasters(users) and broadcastees from different countries for various length of videos. \gareth{We need to explicitly separate the two bars in Figure~\ref{fig:acces_country_based}. Also, we need a takehome for the short vs medium vs long (otherwise there is not point in presenting it). We should also order the bars monotonically, so readers can easily see the rank}}
%%\label{fig:acces_country_based}
%%\end{figure}
%
%%\begin{figure}[htb]
%%%\vspace{-1.5em}
%% \centering
%%\includegraphics[width=1\linewidth]{figs/v2/bcastr_bcastee}
%%% \subfloat{\includegraphics[height=0.4in]{figs/cmap}} 
%%%\vspace{-1.5em}
%%\caption{Fraction of broadcasts of each category on a per-country basis. \gareth{Legend is broken}}
%%\label{fig:cat_distrib}
%%\end{figure}
%
%
%
%%\begin{figure}[htb]
%%%\vspace{-1.5em}
%% \centering
%%\includegraphics[width=0.95\linewidth]{figs/v2/page_gen_vid_distrib_4_sample}
%%% \subfloat{\includegraphics[height=0.4in]{figs/cmap}} 
%%%\vspace{-1.5em}
%%\caption{\% of broadcasters(pages) and broadcastees from different countries for various length of videos. \gareth{We shouldn't have the bars with different sizes - it makes it impossible to compare categories across countries (which is the purpose of the graph). We've already shown the percentage of contribution per country in Figure \ref{fig:acces_country_based} so there's no need to show the same info twice.}}
%%\label{fig:cat_distrib}
%%\end{figure}
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{How far away are viewers?}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%Although the above reveals the locations of broadcasters and viewers, it does not show their relationships. From a systems-perspective, this is critical for optimising delay-\emph{in}tolerant communications as ideally viewers, broadcasters and any intermediate servers would be within short distances. Regarding the latter, there have been a number of recent proposals regarding the placement of servers within cell towers and local network PoPs, \ie so-called mobile edge computing\ns{~\cite{X,X,X}}. Thus, we next inspect the distance that viewers are from the broadcasters they watch. Figure~\ref{fig:vship_dist_cwise} presents CDFs of the distance between broadcasters and their viewers for user accounts. We separate broadcasters into their respective countries. In cases where the distribution plateaus, typically the broadcasters and viewers are separated by an ocean (\eg in the case of Philippines this is the distance across the Pacific to reach US-based viewers, who constitute 9\% of the country's audience).
%
%It can be seen that a notable subset of broadcasters are hyper-local to their consumers. 
%This is shown well in Figure~\ref{fig:local_consumers}, which presents a heatmap of viewer locations relative to the broadcasater. 
%Overall, 8\% of viewers are within 25 KM of the broadcaster and constitute a city-level locality. %In fact, for XX\% of broadcasters, \emph{all} viewers we observe are within this range \ar{given that FB is not showing the locations of all the users, this claim might not be valid?}\gareth{I've adapted the phrasing} \ar{this is actually 0\%, the min such case is 50km. so removing this}. 
%South Korea is the most extreme in this regard; 11\% of viewers are within 25KM, with 4\% actually under 5KM. We can also inspect the opposite end of the spectrum. 11.35\% of viewers are over 10,000 KM away from their broadcaster. Here, subtle differences can be seen between broadcasters from different countries. For example, broadcasters from the Philippines tend to be further away from their viewers (only 37.81\% of viewers are closer than 1000 KM), whereas Turkish broadcasters generally garner more nearby viewers (52.71\% are closer than 1000 KM). 
%
%\begin{figure}[th]
%	%\vspace{-1.5em}
%	\centering
%	\includegraphics[width=1.0\linewidth]{figs/v3/cell_wise_viewers.pdf}
%	\caption{Number of viewers (binned at 500m) within a radius of 5KM, 25KM and 40KM when all the broadcasters location are shifted to origin.}
%	\label{fig:local_consumers}
%\end{figure}
%
%As previously discussed, this local content consumption suggests that live social streaming would be well placed to benefit from technologies such as mobile edge computing.%, where services can be placed directly into cell tower. \ns{ This 35KM assumption sounds a bit weak. Aravindh, can you dig up something about cloud RAN and micro data centers? We can probably get away with a micro data centre that serves a few cities... Or some kind of national or regional infrastructure.} If we assume a cell tower range of 35 KM\footnote{This is the upper range for GSM???????}, we find that XX\% of broadcasts could exclusively be served within the range of a single cell. \gareth{Could we beef up this style argument? Maybe have a graph that shows how much we can localise based on different cell ranges?} \ns{This sounds like a good idea.}
%%\ar{wouldn't this be similar to fig 11(a)?}
%%\gareth{Haha, think the fig reference is out of date, so I'm not sure which fig 11a is. I'm guessing fig 9 nowa? But I don't think we have this style of fig yet. Basically, each line would represent a cell range, e.g. 1KM, 5KM, 10KM etc. Each line would then be CDF that captures the fraction of viewers (per broadcast) that can reach their broadcaster within that range. It's similar to fig 9 but will make the ``cell'' message much more clear.}
%
%
%
%
%%\begin{figure}[ht]
%%%\vspace{-1.5em}
%% \centering
%%\includegraphics[width=0.95\linewidth]{figs/v2/broadcastee_dist_pg_us}
%%% \subfloat{\includegraphics[height=0.4in]{figs/cmap}} 
%%%\vspace{-1.5em}
%%\caption{ Where the video broadcast made by user/page is watched. }
%%\label{fig:broadcastee_dist_pg_us}
%%\end{figure}
%
%%\includegraphics[width=0.95\linewidth]{figs/v2/vship_dist_cwise}
%% \subfloat{\includegraphics[height=0.4in]{figs/cmap}} 
%%\vspace{-1.5em}
%\begin{figure*}[thb]
%%\vspace{-1.5em}
% \centering
% \subfloat{
% 	\label{fig:vship_dist_cwise}
% 	\includegraphics[width=.32\linewidth]{figs/v3/dist_counts}
%	}\hfill
% \subfloat{
%	 \includegraphics[width=.35\linewidth]{figs/v3/char_1}
%	 \label{fig:mob_consumption}
%	}\hfill
% \subfloat{
%	\includegraphics[width=.29\linewidth]{figs/v3/prod_cons_all_2}
%	\label{fig:coun_heatmap}
%	}
%\caption{Geographical footprint: \protect\subref{fig:vship_dist_cwise} CDF of distance between broadcasters of their viewers. Multiple plots are presented for broadcasters in different countries
%\protect\subref{fig:mob_consumption} Fraction of views from users in the same country as the broadcaster
%\protect\subref{fig:coun_heatmap} Fraction of views from users in a \emph{different} country from the broadcaster, shown as a heat map of content broadcast from one country consumed in another country, plotted for the union of top 15 producers and consumers.
%}
%
%\end{figure*}
%
%\subsection{Domestic or international?}
%
%
%
%It should be remembered that distance can be deceptive due to the various sizes of individual countries. Since we expect infrastructure to be confined within country borders, we next separate all broadcasters and viewers into their respective countries. Figure~\ref{fig:mob_consumption} presents the fraction of the views for videos of a country which come from domestic viewers. This is computed as follows: For a given country, we take the total view count of all videos broadcasted from that country. We present the \emph{fraction} of these views that are domestic, i.e., from viewers in the same country as the broadcaster.  In some cases (\eg Thailand, Vietnam), over 80\% of views are  domestic, suggesting strong language, social and cultural ties drive consumption. In other cases, under 20\% of viewers are domestic (\eg Germany). This suggests such countries generate highly popular international content. However, we note that almost all videos have a non-trivial local viewership; and thus would benefit from caching locally in the country of broadcast, regardless of whether the video also has an international appeal or not.
%
%To explore the international views, Figure~\ref{fig:coun_heatmap} presents a heat map of the \emph{non-domestic} views. Each cell in the matrix represents the fraction of views for videos of a country which come from a specific consumer country. For the sake of clarity, the fraction of domestic views (where the producer and consumer are from the same country) are not plotted. Further, only the top 19 producers and consumers are shown; thus the fraction of the heat map values across all consumers might not add up to 1. 
% It can immediately be seen that a small number of countries stand-out in regards to the global reach of their content. The US is most prominent, with a particularly large build-up of viewers in Mexico and Canada. This is not surprising considering the high degrees of immigration and cultural overlap between these three countries. \ar{cite?} Despite our prior observation about local consumption, Thailand and Vietnam also have a large number of viewers from other countries. 
% %This number is large, relative to the global audience for videos from other countries. In absolute numbers, these foreign viewers constitute under 20\% of the audience.\gareth{Could these last 2 sentences be clarified, not sure the message is clear}
%  Much like the US, this is driven by the large number of broadcasts in the country. Manual inspection reveals that many of the global views are for videos of a risqu\'e or adult nature. 
%  
%   
%  Before concluding, we note that Figure~\ref{fig:coun_heatmap} is merely intended to illustrate some interesting international trends and is not a complete picture -- for instance, countries like DE and TR, which have a high proportion of non-domestic views (Figure~\ref{fig:mob_consumption}) do not show up with high values in this heat map because the consumers for the vidoes broadcasted from these countries are not amongst the top 19, and hence are not shown.
%
%
%% 
%
%
%%
%%\begin{figure}[ht]
%%%\vspace{-1.5em}
%% \centering
%%%\includegraphics[width=0.95\linewidth]{figs/v2/producer_consumer_v4} \
%%\includegraphics[width=1\linewidth]{figs/v3/prod_cons_all_1}
%%%  \subfloat[Page Broadcasts]{\includegraphics[width=0.30\linewidth]{figs/v2/producer_consumer_2_pg_bcast}}\
%%%  \subfloat[User Broadcasts]{\includegraphics[width=0.30\linewidth]{figs/v2/producer_consumer_2_us_bcast}}
%%% % \subfloat{\includegraphics[height=0.4in]{figs/cmap}} 
%%%\vspace{-1.5em}
%%\caption{ Heatmap showing the fraction of content broadcast from one country that is consumed in another country (plotted for the union of top 15 producers and consumers). It shows that almost 50\% of content is consumed locally within the nation.}
%%\label{fig:producer_consumer}
%%\end{figure}
%
%
%%We also briefly note that the ability to perform such analysis could expose users to privacy violating attacks. Although viewer names are not listed with coordinates, in some cases it would be trivial to geolocate specific users. For example, users who leave comments immediately reveal themselves as viewing a video. If an attacker knew the city of residence for the user, this could be used to extract any coordinates that fell within the appropriate polygon. We find that XX\% of broadcasts have an entire set of viewers who are at least 10KM apart --- in such cases, a privacy-compromising attacker could easily exploit this information.
%
%
%%\subsection{Distance \vs Duration?}
%%Considering the trend for users to consume content from their own countries, we are curious to see what characteristics define a stream that is consumed outside of its own country. As a first step, Figure~\ref{fig:viewership_across_time} presents the minimum distance a broadcaster is from its viewers based on the duration of the broadcast (for a number of countries). It can be seen that the minimum distance of viewers increases as the duration of the broadcast increases. Despite the similarity across countries, it can be seen that the incline for countries like TH are far less than for counties like US or Brazil....
%%\begin{figure*}
%%\vspace{-1.5em}
% %\centering
% %\subfloat[US]{\includegraphics[width=0.24\linewidth]{figs/v2/viewership_across_time_us}}
% %\subfloat[TH]{\includegraphics[width=0.24\linewidth]{figs/v2/viewership_across_time_th}}
% %\subfloat[VN]{\includegraphics[width=0.24\linewidth]{figs/v2/viewership_across_time_vn}}
% %\subfloat[BR]{\includegraphics[width=0.24\linewidth]{figs/v2/viewership_across_time_br}}
%% \subfloat{\includegraphics[height=0.4in]{figs/cmap}} 
%%\vspace{-1.5em}
%%\caption{How viewership changes across time during the broadcast of the video. X-axis indicates the $n^{th}$ minute of video and y-axis indicates the minimum distance at which an user is watching the video. \gareth{Maybe worthwhile playing with some other Y metrics for Figure~\ref{fig:viewership_across_time}, e.g. median/mean/max. Also, all graphs show broadly the same trend. Were there any countries where the trend was very different?}}
%%\label{fig:viewership_across_time}
%%\end{figure*}
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%% \begin{figure*}
%% %\vspace{-1.5em}
%%  \centering
%% \subfloat[Arts \& Entertainment]{\includegraphics[width=6in]{figs/v1/pagewise/Arts_Entertainment_dissem.png}} \
%% \subfloat[Outdoor, Recreation \& Fitness]{\includegraphics[width=6in]{figs/v1/pagewise/Outdoor_Recreation_Fitness_dissem.png}} \ 
%% \subfloat[Public \& Government Services]{\includegraphics[width=6in]{figs/v1/pagewise/Public_Government_Services_dissem.png}} \\
%% \subfloat[Locality]{\includegraphics[width=6in]{figs/v1/pagewise/Locality_dissem.png}} \
%% \subfloat[Religious Place of Worship]{\includegraphics[width=6in]{figs/v1/pagewise/Religious_Place_of_Worship_dissem.png}} \
%% \subfloat[Media]{\includegraphics[width=6in]{figs/v1/pagewise/Media_dissem.png}} \
%% \subfloat[Shopping \& Retail]{\includegraphics[width=6in]{figs/v1/pagewise/Shopping_Retail_dissem.png}} \
%% \subfloat[Other]{\includegraphics[width=6in]{figs/v1/pagewise/Other_dissem.png}} \
%% % \subfloat{\includegraphics[height=0.4in]{figs/cmap}} 
%% %\vspace{-1.5em}
%% \caption{ category wise (top-6) content access across the globe indicating localisation of content production and consumption. List of categories available at: \url{https://gist.github.com/arvyram/b6f912f4ec8544470922fbb18ead873c}
%% }
%% \label{fig:cat_wise}
%% \end{figure*}

==> sections/figdump.tex <==
\section{Added to the Story}

\subsection{\ns{Q-R1. Literature Survey Edits} Readings Reference from Todd Graham, Andres Jungherr and Darren Lilleker}\label{sec:survey}

\ew{Ans: Added by Edward}

Earlier studies mostly relate to a period when the use of Twitter by UK politicians was in its infancy, with a small fraction being regular users~\citep{jackson2011microblogging, lilleker2013online, graham2013between, graham2016new}.  Nevertheless, there were early indications that use of Twitter was entering the mainstream of electoral campaigning and political communications generally. Although, political tweets might not look like substantive \emph{contributions} to the political discourse, they appear to have become \emph{an increasingly integrated element of political communication in a `hybrid media system'} ~\citep{jungherr2016twitter,jackson2011microblogging}.

~\cite{jackson2011microblogging} identified three ways in which UK MPs used Twitter: impression management, constituency service and regular communications. ~\cite{lilleker2013online}, in a study of members of the European Parliament, developed this typology to cover homestyle (highlighting the work and achievements of the member to demonstrate active service to those they represent) and participatory communications in addition to impression management.  Characteristics like gender, party and seniority of the participating MP were associated with different communication styles.

One-way communications(``broadcasting'') predominated ~\citep{graham2013between,jackson2011microblogging,lilleker2013online}, but participatory communication through Twitter was seen to be emergent.  It seemed to fit neatly into ~\cite{coleman2005blogs} concept of direct representation ~\citep{graham2013between} and politicians talked about their use of Twitter in these terms, but it was still secondary to other uses ~\citep{jungherr2016twitter}.  Nevertheless, ~\cite{graham2013between} found that 19\% of candidates' tweets during the 2010 general election campaign interacted in one way or another with voters, which they argued was a fairly substantial level of interaction compared to other forms of political communication during the campaign.  A participatory style of communications on Twitter had potential to earn legislators political capital ~\citep{jackson2011microblogging} and was the only statistically significant strategy that had a positive impact on the size of the community ~\citep{lilleker2013online}.

Cross-party communication between MPs was found to be unusual.  Unsurprisingly, MPs indulged in one-off attacks on other politicians during the 2010 UK general election campaign ~\citep{graham2013between} but there was evidence of a more collaborative approach amongst an ``organic community'' of early adopters on Twitter~\cite{jackson2011microblogging}. Supporters of different parties tended to cluster around different hashtags during election campaigns, creating politically separated communication spaces ~\citep{jungherr2016twitter}. 

\pa{Ans: Summary by Pushkal}
\begin{itemize}
\item ~\cite{jackson2011microblogging} ``Microblogging, constituency service and impression management: UK MPs and the use of Twitter.'' The Journal of Legislative Studies 17.1 (2011): 86-105. [218 cites]

MP do engage with the online platforms where certain characteristics like gender, party and seniority of the participating member impacting on this behavior. \emph{Impression management(Ingratiation, Self-promotion, Supplication, Exemplification and Intimidation)} is the primary goal of doing this and \emph{constituency service} as secondary. The former itself gives an intuitive picture of the leader to the general audience, plausibly the voter from their constituency. Promoting party agenda MPs act as cheerleaders for their political parties. To some extent constituency service has also given credits to a leader by being a welfare officer and local promoter.  

Pros- Interesting facts and methodology for finding scores of impression management and constituency service.
Cons- Current Twitter space has been changed. Almost all the MPs are on twitter with party, self and local promotions and arguments.

\item \cite{lilleker2013online} ``Online political communication strategies: MEPs, e-representation, and self-representation.'' Journal of Information Technology and Politics 10.2 (2013): 190-207. [58 cites]

Extension of parts of work in~\cite{jackson2011microblogging} by introducing three kind of strategies used by MEPs (Member of European Parliament). First is homestyle which refers to allocation of resources or propagating messages already published. Second and thirt i.e. impression management and participatory are same as~\cite{jackson2011microblogging} , where the latter was coined as constituency service.
Pros- MEPs are from different nations and hence they represent, work and engage with their residing nation more.
Cons- MEP are elected from a bigger area. From 2014-19's MEPs list, 73 in 751 are from UK. This would lead to disengagement. People hardly know who is their MEP.    

\item ~\cite{graham2013between} ``Between broadcasting political messages and interacting with voters: The use of Twitter during the 2010 UK general election campaign.'' Information, Communication and Society 16.5 (2013): 692-716.[220 cites]

Some politician do believe in online interaction while some use only for one-way communication. In 2013, nearly two-third of MPs were active on popular social networking site, Twitter. Twitter became a new online space for bi-directional interaction unlike exiting websites and wikipedia pages for almost a decade. This paper analyses for type of tweets posts- normal,@-reply, retweet and comment. Data was taken from 2010 Uk general elecitions competing politicians and All @-reply are \pa{labeled for one of twelve type of person, tweets for fourteen functions and topic in nineteen categories.} Conservative were more interactive with public and posting more normal posts. Labor was more engaging with party activists and putting more replies.
Pros- Possible overlapping work for extending interaction patterns. 
Cons- Election time is a focused period with different moods and strategies. Only 26K tweets observed.

\item ~\cite{graham2016new} ``New platform, old habits? Candidates' use of Twitter during the 2010 British and Dutch general election campaigns.'' New media and society 18.5 (2016): 765-783.[115 cites]

An extension of [Graham 2013, ``Between Broadcasting...''] with more or less same content and figures

\item ~\cite{jungherr2016twitter} ``Twitter use in election campaigns: A systematic literature review.'' Journal of information technology and politics 13.1 (2016): 72-91. [114 cites]

This is a survey of 127 election study papers from Twitter space. Though interesting but they proposed this as an orthogonal study from regular interaction analyzing papers and outside the election period.

\item ~\cite{butler2001payment}``Payment on delivery-Recognising constituency service as political marketing.'' European Journal of Marketing 35.9/10 (2001): 1026-1037.[98 cites].

Taken political engagement as a marketing scheme and arguing that it worths only 500 votes~\citep{norton1990constituency}. Taking political campaign as a permanent phenomenon, the daily services to citizens by politicians are hard to do but a general and regular constituency service, assessment, planning and election consideration is throughout the tenure. 

\item ~\cite{auel2018explaining} ``Explaining MPs' communication to their constituents: Evidence from the UK House of Commons.'' The British Journal of Politics and International Relations (2018): 1369148118762280.

This paper talks about the MPs communication with respect to the constituents, single way and during non-election period. The purpose of doings so is to observe trustworthiness developed with re-election prospect(majority winner,senior, not electing next time are lazy), constituency characteristics (urban and far from parliament are more engaged) and legislature behavior(votes in parliament, party line, marginal rebels).  

\item ``From everyday conversation to political action: Talking austerity in online ‘third spaces’'', Graham and Jackson 2015, \url{http://journals.sagepub.com/doi/pdf/10.1177/0267323115595529} Analysing www.netmums.com, www.digitalspy.com and www.moneysavingexpert.com. This paper takes data from 3 websites and claims that 50\% of which has motivated political actions.

\item ``Interactivity and Political Communication: hypermedia campaigning in the UK, lilleker 2015'' Using web 2.0 for political communications(party, campaign, etc). Disparity in strategies and collective activity measures are presented.

\item ``Elite Tweets: Analyzing the Twitter Communication Patterns of Labour Party Peers in the House of LordsAna Adi, Kristofer Erickson, and Darren G. Lilleker (2014)'' Tweeting behavior is consistent among communities. Labor people work in small groups.

\item Lilleker, Darren G., and Karolina Koc-Michalska. "What drives political participation? Motivations and mobilization in a digital age." Political Communication 34.1 (2017): 21-43. Explaining intrinsic and extrinsic nature of online political communication the authors also studies motivations of use of non-conventional digital media.   

\item Latest papers by Lilleker focuses on citizen engagement in cases like \emph{campaigns, media sharing, EU/spain elections}. These works mostly consider what citizen are saying online.

\end{itemize}

\ew{Ques from edward: In general, how far are the bursts the result of conscious communications plans, or are they more to do with luck and opportunism? How much do we know about how the bursts start? We know that in some cases it's to do with a minister resigning, being sacked or being appointed. But do we know about enough of the bursts to identify a typology?}
\pa{Ans: TBD}

\subsection{Constituency Service and Mentioners}
\ns{Q-R2: What are the non-legislators' account? Politicians, public figures or residents.}
\pa{Ans: We analyse non legislators for their Constituency and botness score. We found that although people focus on their elected MPs but MPs focus on constituents is almost zero[TBA more]. Moreover, we already discussed in ``Conversation of MPs'' that MPs interact with UK residents, to people they follow.}

\subsubsection{Constituency Focus}
To Be Added (today)
\pa{Got Idea of adding more geo-tagged data. Updating soon location matched with postcodes using Twitter Profile location(25,000 Postcode tweets of UK). This will also update constituency focus as 500 reply and Rt are given to mentions from the constituency.}

From all $\Leftarrow$ we found 54K geo-tagged tweets [To Be Added: and 80K RT and 15K reply from $\Rightarrow$ are given to $\Leftarrow$, checking user profiles location postcodes now, got 25K Postcodes and non zero constituency focus] and for the same we discovered the postcodes using \emph{photon} library in R. The UK consists of around 2.5 Million postcodes\footnote{\url{https://www.doogal.co.uk/UKPostcodes.php}}, we took list of the same which provides postcodes in a constituency. Another method could be using parliament services via link \footnote{\url{http://www.parliament.uk/mps-lords-and-offices/mps/?search_term=<POSTCODE>}}. The latter could be helpful for finding small number postcode linked to MP's page. 

Interestingly, we found that although for $\Leftarrow$ some ``focus'' exists to MPs from their constituencies (shown in Fig.~\ref{fig:geoFocus} ) but form the $\Rightarrow$ we find almost zero[not for profile located now] instances corresponding to those constituency posts. Among all the MPs we only find one reply and two retweets given to constituency mentions. This relates to popular theory of which says constituency service worth only 500 votes. MPs hardly attend and respond to online query and in turn to constituency service is still not prevalent. 

\begin{figure}
\vspace{-0.5cm}
      \begin{center}
		\includegraphics[width=.9\columnwidth]{figs/CDFGeoIN}
		\caption{Constituents focus for $\Leftarrow$. Some MPs do get high ``focus'' of mentions from their constituency. These are mostly not so popular MPs who are hyper-locally engaged.}
		\label{fig:geoFocus}
		\end{center}
\vspace{-0.5cm}
	\end{figure}

\subsubsection{Botness}\label{sec:botCheck}
All $\Leftarrow$ tweets were analyzed for being a Bot or not. In online platforms bot are automated accounts which are set up using APIs. For this purpose we computed bot scores of all the $\Leftarrow$ users using Botometer~\citep{davis2016botornot,varol2017online}\footnote{\url{https://osome.iuni.iu.edu/}} developed, maintained and regularly improved by Indiana university researchers. 
Bot detection is also run by Twitter, the algorithm of which is frequently updated. As per~\cite{chavoshi2016debot}, generally Twitter platform takes three months for bot checking and then suspected account are deleted.~\cite{Zhong:2014:SBP:2566486.2568031} claims that deletion of accounts are mostly suspected as fake. Results for the health of our data are in Tab.~\ref{table:botCount}. 
The latest check for deleted accounts from our data is done in August 2018, roughly after nine months of the actual dataset period. This allowed three sprints for internal Twitter bot checking. Also, during the period of May to July 2018 Twitter did major sanitation check which resulted in suspension of 70 million account worldwide. \footnote{\url{https://www.nytimes.com/2018/07/11/technology/twitter-fake-followers.html}} and official report\footnote{\pa{break line \url{https://blog.twitter.com/official/en_us/topics/company/2018/how-twitter-is-fighting-spam-and-malicious-automation.html}}}. The top fifteen UK MPs losing followers on $13^{th}$ July 2018 are shown in Figure~\ref{fig:botdeleted}, where Boris Johnson lost almost 30K followers. Also, the bot score obtained for all the $\Leftarrow$ users is given in Fig.~\ref{fig:TopBot}

\subsubsection{Mentioners}
~\cite{graham2013between} categorized MPs interactions with one of \emph{Public, Politician, Journalist, Party Activist, Lobbyist, Expert, Celebrity, Industry and Authority} person. This was done for UK 2010 elections time data. We coded MPs replies and retweets to citizen, other party MPs, followings and residence(hereafter constituents). 

\begin{table}
\vspace{-0.1cm}
\centering
 	\begin{tabular}{|p{1.9cm}|p{1.2cm}|p{1.7cm}|p{1.7cm}| } 
		\hline
		User Type&Users& $\Leftarrow$ Activity& $\Rightarrow$ Activity\\
        \hline
        Protected&4,677&30,042&610\\
        Deleted&16,386&170,899&1,906\\
        Bot Detected&17,141&75,238&12,413\\
        Others&234,186&1,893,559&85,650\\
         \hline
	\end{tabular}
    \caption{$\Leftarrow$ Activity by different(272K) types of users' accounts. Also, $\Rightarrow$ Activity by MPs towards these users. For Bot Detection Botometer Score of more than or equal to 0.5 is considered. Interestingly, deleted account were having high activity during study period of attention. The same deleted accounts also got $\approx$2000 replies and retweets from MPs.}
		\label{table:botCount}
\end{table}

\begin{figure} 
\vspace{-0.1cm}
		\begin{center}
		\includegraphics[width=.9\columnwidth]{figs/botsDeleted}
		\caption{By $13^{th}$ July many bots were deleted from Twitter resulting a negative new follower count for half of the MPs.}
		\label{fig:botdeleted}
		\end{center}
        \vspace{-0.5cm}
	\end{figure}

\begin{figure}
		\begin{center}
		\includegraphics[width=.9\columnwidth]{figs/botometer}
		\caption{Botometer Score for 188K users from $\Leftarrow$ activity user. ~1\% Protected accounts,
3.8\% Deleted accounts, 50\% are having $<$0.3 Bot score
and 9,212 (~5\%) users are having $>$ 0.5 Bot Score\pa{check unique scores}}
		\label{fig:TopBot}
		\end{center}
        \vspace{-0.5cm}
	\end{figure}



\subsection{Staff Management coding scheme}
\ns{Q-R2: Interpretation and implications of staff management}
\pa{Ans: We explored Twitter status source and variability in MPs device usage. Also, staff managed activity is know to cause high bot score and follow different linguistic and temporal features.}

\subsubsection{Twitter Status Source}
To explore the ``use'' of Twitter by MPs or by their staff we explored a best possible case of \emph{Twitter status source} provided by Twitter API for each tweet which is posted. These statuses refer to \emph{mobile device, desktop application or third party} authenticated sources (\eg TweetDeck, Alex Cunningham MP Websites 2017, Twitter Ads, Instagram and so forth). A `word cloud' is presented in Fig.~\ref{fig:statusCloud} where size of `word name' is proportional to the `frequency' in all $\Rightarrow$ activity. The same word cloud be created for $\Leftarrow$ but not presented here due to limited space and also some overlapping ideas are already covered in Bot or not, Sec.~\ref{sec:botCheck}.

Also, exploring Twitter status source we counted each source's \emph{reply, retweet and posting} activity from MPs. In total we found 47 and out of all the sources, 98\% data are covered in \emph{seven} sources given in Fig.~\ref{fig:statusRtRp}. Apart from that few platforms like instagram, facebook and MPs website share posts as cross platforms, such type of sharings falls under posting only. \emph{The Atlantic}\footnote{\url{https://www.theatlantic.com/politics/archive/2017/03/a-bot-that-detects-when-donald-trump-is-tweeting/521127/}} published insights in a news article where US President `Donald Trump's' (current US President) Twitter account was analyzed for his personal and staff managed tweets. Donald Trump was using `Android' phone in his early days after becoming the President but still some tweets were from iPhone. This provided some data to the analysts for considering iPhone activity staff managed tweets. Later, they developed a classifier \footnote{\url{ https://github.com/arm5077/trump-twitter-classify}} and found variation in @,\#,"", and so forth linguistic characteristics which differs and proves to be 90\% accurate in labeling President and staff tweets. Use of multiple devices (as tweet source) could corresponds to multiple people managing a same account. In found that replies given by MPs are highly focused to use of one device only than doing other posts Fig.~\ref{fig:sourceFocus}.

\begin{figure} 
		\begin{center}
		\includegraphics[width=.9\columnwidth]{figs/statusCloud}
		\caption{Word Cloud of Twitter Status Sources. There are 47 sources in total. }
		\label{fig:statusCloud}
		\end{center}
        \vspace{-0.5cm}
	\end{figure}
    


\begin{figure}
		\begin{center}
		\includegraphics[width=0.9\columnwidth]{figs/statusRtRp}
		\caption{Exploring Twitter Status source for personal and staff managed tweets. Web based platforms like \emph{Twitter Web Client and TweetDeck} are more used for posting purposes.}
		\label{fig:statusRtRp}
		\end{center}
\end{figure}


\subsubsection{Botness and LIWC}
We also check bot scores of all the MP and found that \emph{forty-five} MPs accounts crosses the threshold of botness. LIWC difference are also evident among mobile based and other post. With LIWC score of all $\Rightarrow$. a major difference is observed among web based and mobile based sources. Web based (Web Client and Tweetdeck) are more related to money, work, uses we and they, puts question mark and mostly focus on present. Moreover, the same platform lacked in anger, female, you pronoun, exclamations and highly lack in informal speech(assent and netspeak) scores.   

\begin{figure}
		\begin{center}
		\includegraphics[width=0.9\columnwidth]{figs/mobiWebLiwc}
		\caption{With LIWC score web based activity is highly formal, focused on present and less social.}
		\label{fig:mobiWebLiwc}
		\end{center}
\end{figure}


\subsection{Comparison With Journalists and among FrontBench MP}
\ns{Q-R2: Why such baselines, and actors interactions are different. Also, are the mentioners? }
\pa{Ans: We found using GWI survey data that MPs and Journalists do have same type of audience. Also a simple case use is a comparison among MPs taking a set of frontbench and rest of the MPs}
\subsubsection{Journalists as Base line}
Using Global Web Index survey data \url{https://pro.globalwebindex.net/}, we validated the similarity in audience which is following MPs and Journalist. We created an audience which consumes digital news content, use social media and recommends/comments on brands on social media. We got 32.5\% and 32.1 as audience \% and almost same universe answering the question for the survey. 
	
\subsubsection{Front Bencher MPs}
Using lists published at parliament.uk\footnote{\url{https://www.parliament.uk/mps-lords-and-offices/government-and-opposition1/}} of government and opposition forming MPs, we found and labeled 96 of 559 names as \emph{Frontbench}. In total 17\% MPs sitting on \emph{FrontBench} have 4.5 Million follower count and correspond to 44\% and only 19\% $\Leftarrow$ and $\Rightarrow$ activities. Frontbench MPs are quite busy! Also, nine front bencher MPs are high on Botometer score. Organizational (here MPs staff) and promotional accounts are being managed by many people and hence classified as Bot~\citep{rizoiu2018debatenight,varol2017online}. Nonetheless, thirty-six non front bench MPs are also high on Botometer check. Difference $\Leftarrow$ and $\Rightarrow$ is already presented with baseline \pa{updated focus CDF in Fig.~\ref{fig:mentionsActivitiesFBJ}, removed actors with Frontbench and Other MPs from Fig.~\ref{fig:mentions-activities}.} The median of attention (focused) days is four days for \emph{FrontBench}  MPs while for others is five days. Also, the former mostly user iPad for posting after iPhone while in the latter the second choice is changed to Android.

\begin{figure}
   \vspace{-0.5cm}
	\centering
	\includegraphics[width=0.49\columnwidth]{figs/mpMentionFBJ.pdf}
   	\includegraphics[width=0.49\columnwidth]{figs/mpActivityFBJ.pdf}
	\caption{Frontbench MPs vs.\ Other MPs vs.\ Journalists. Left: Cumulative Distribution Function (CDF)\footnote{The further to the right a CDF curve is, the larger the value of the variable it is tracking}. of the number of mentions received by users in each category, showing that frontbench MPs receive more mentions other MPs and Journalist. Right: CDF of the number of actions  (Tweets+Retweets+Replies) on the ``Tweets and Replies'' timeline of the user, showing that all MPs produce more timeline actions than journalists. @CGreenUK conservative frontbench MP and @khalid4PB Labour other MP have highest actions in their category.}
	\label{fig:mentionsActivitiesFBJ}
\end{figure}

\subsection{Interactions and Cases}
Among user who are in $\Rightarrow$, not all follow MPs. Interestingly, from these 66.17\% follows at least one MP. Total unique followers are 4.28 Million with median MPs followed count as 3.


\ew{\subsubsection{Twitter as a channel for public consultation on legislation}
	Individual MPs in the UK Parliament are able to submit Bills (draft legislation).  These are known as Private Members' Bills.  Priority is given to Government-sponsored Bills, so to ensure that a proportion of Private Members' Bills have a chance to become law there is a ballot of MPs each year to assign priority for the limited amount of debating time available.  Even Bills coming high up in the ballot are unlikely to be passed unless they have the tacit or explicit support of the Government.
	Chris Bryant, a Labour back bench MP, came top in the ballot for the 2017-19 session.  He launched a consultation on Twitter, putting forward six possible Bills and asking Twitter users to choose their favourite.  45,000 people participated \footnote{Source: \url{https://www.youtube.com/watch?v=RqkSSQ3bAaA}} and the winner was a proposal to provide additional legal protection to emergency service workers, as a result of reports of assaults by members of the public during emergency call-outs.  Bryant introduced the Assaults on Emergency Workers (Offences) Bill 2017-19, which was supported by the Government.  Tweets during the passage of the Bill through Parliament enabled the public to comment (as well as garnering publicity for Bryant).  There were calls to extent the scope of the Bill, for example: \url{https://twitter.com/rhonddabryant/status/930811632707653638}.
	The Bill received Royal Assent, the final stage on the way to becoming a law, on 13 September 2018.}


\subsubsection{Chris Bryant survey, thanking and video on Twitter while proposing his Bill}


\subsubsection{Snapshots of Cases}
Argumentation case in Fig.~\ref{fig:davidLammy}
\begin{figure}	
		\begin{center}
		\includegraphics[width=\columnwidth]{figs/davidLammy1July}
		\caption{Tottenham MP David Lammy replied to a comment which questioned his support to remain in EU. Although the mentioner deleted his tweet but the MP then shared the snapshot (on right) of the same comment with a thanking reply. }
		\label{fig:davidLammy}
		\end{center}
	\end{figure}
Other MPs engagement clip are in Fig.\ref{fig:interactions}.

\begin{figure}	
		\begin{center}
		\includegraphics[width=\columnwidth]{figs/mpsInteracting}
		\caption{Top-left, MP Amber Rudd after resignation tweet addressed to the new minister. Bottom-right, Prime Minister Theresa May thanking for event. Right, Damian Collins on his review after select committee meeting.}
		\label{fig:interactions}
		\end{center}
	\end{figure}


Also, an example of ``new'' (and in development) ways on interacting is Matt Hancock's mobile APP.     \footnote{\url{https://www.theguardian.com/world/2018/mar/22/minister-forced-to-change-his-own-app-after-data-mining-complaints}}

\subsection{Temporal patterns, availability}
\ns{Q-R3: Temporal patterns and availability.}
\pa{Ans: We found daily activity and compared sources Figure~\ref{fig:weekActive}} 

Web based activity is decreased during weekends whereas twitter web client is the highest \% active source on most active day, \emph{Wednesday}. \ew{Why Wednesday?}

\section{\pa{Question In Mind}}
\begin{itemize}
\item Coding of mentioners?
\item How far to present burst?
\item Wednesday high $\Rightarrow$?
\item Case Studies?
\item `Tense' to follow/change will writing papers.
\end{itemize}



==> sections/relatedWork.tex <==
\section{Related Work}


%As Internet access has spread, studies by \cite{groshek2009democratic,rhue2014digital} and others have looked at the effect the Internet has had on democracy in general. \cite{groshek2009democratic} was a pioneering cross-national study of 152 countries that showed that Internet access was positively associated with diffusion of democracy. More recently~\cite{rhue2014digital} demonstrated that mobile penetration contributes even more than Internet access to the spread of democracy. 

A large part of the influence social media has had on the democratic process has been as a tool to organise protests, such as the Arab Spring revolution~\citep{tufekci2012social,gerbaudo2012tweets},  Occupy Movement~\citep{fuchs2014occupymedia} and Los Indignados~\citep{theocharis2015using} movements, etc. A second aspect that has received considerable attention is the role of social media in the elections, in UK~\citep{anstead2015social,ahmed2016tweets}, USA~\citep{cogburn2011networked}, India~\citep{belair2015verdict2014,ahmed2016tweets}, Italy, France etc.~\citep{ceron2014every}. %Especially in the context of elections, there has been an interest in predicting election results~\citep[e.g.][]{o2010tweets,tumasjan2010predicting}, but also some caution about the difficulties due to the non-representative nature of social media active users and limited availability of accurate profile and demographic information~\citep{metaxas2011not}. 
In contrast with such works, we are interested in understanding  discourse between elected representatives on the one hand, and citizens and other Twitter users on the other, during ``normal'' times, when there is no incipient change of power due to election or revolution.

Several~\citep{shirky2011political,mossberger2007digital,rotman2011slacktivism,loader2011networking,bimber2017three,wells2015civic} have looked at how citizens can contribute, organise themselves, and express opinions on elected representatives and other democratic issues using digital and social media tools. Our work looks at the other side of the conversation -- how MPs engage with Twitter users --  and therefore is complementary. However, looking at the role of the citizen in online democratic conversations is important to help give a context to our work.  Some, especially early works such as~\cite{mossberger2007digital} saw economic opportunity, civic engagement and online participation as important benefits for citizens who use online platforms. Similarly, \cite{shirky2011political} saw  social media as  ``long term tools that can strengthen civil society and the public sphere'' and posited that access to conversation is more important politically than access to information. However, there have been debates about whether citizens engaging  on social media is merely `slacktivism'~\citep{rotman2011slacktivism,slactivism-cacm}. Yet others, such as \citep{loader2011networking} argue for a cautious approach, suggesting that the definition of what it means to `participate' in a democracy should be expanded, if social media activity should be included as participation in a democracy.  \cite{bimber2017three} propose that the digital media environment should be seen as a change in the context for action. \cite{wells2015civic} makes the case that a shift in information styles may help to explain the disjuncture felt by many young people when it comes to traditional institutional participation and politics. 


%An important part of the wider background and context is work on how political communication on social media can be used to  mislead civic society, for instance through astroturfing, Twitter Bombs, bots etc.~\citep{metaxas2012social}. As a case in point, \cite{allcott2017social} paint a picture of the economics behind fake news and its propagation in relation to the recent 2016 US Elections. While such possibilities are important to keep in mind, studying these are outside the scope of (and orthogonal to) the current work. We believe that there was no large-scale misinformation campaign conducted on the UK political conversation in Twitter during the dates of our study.

Closest to our work are studies done both in the offline and online contexts about how MPs engage with their constituents. There has been considerable work over the years in the offline context. For example,~\cite{krasno1997challengers} talks about the `incumbency factor' and the need to develop this relationship in order to get re-elected. ~\cite{stanyer2008elected} suggest that MPs' engagement with constituents has recently been changing, and identifies four ways in which MPs relate to their constituents: through casework (helping individuals with specific govt problems), projects (helping groups with their efforts), gaining visibility (by highlighting work they have done), and party maintenance (spreading the message of their Political Party). 
\cite{butler2001payment} studies MPs' engagement with their constituents as political marketing, and calculates that local service is worth about 500 votes. 

Work on the use of digital media by elected representatives, especially MPs in the UK, has been pioneered by Jackson, Lilleker and others. \cite{ward2003line,jackson2004just} looked at the use of websites by election candidates and MPs. \cite{coleman2005blogs} says blogs by UK MPs should be considered as listening posts for political signals rather than as platforms for one-way communication. \cite{jackson2008representation} follow up on this work by interviewing 4 UK MPs, and find that blogging leads to an e-constituency that competes with the geographic constituency for the time of the MP.  

Amongst other studies, \cite{jackson2011microblogging} was an early look at MPs on Twitter, using content analysis with manual coding. In contrast we take a more quantitative approach that allow us to scale to millions of Tweets and mentions. Such an approach is necessitated by the drastic shift from 2011, when ``only a small group of [51] MPs [used] Twitter as a regular communication channel, but most [were] only occasionally dipping their toe into the microbloggersphere'' to now, when nearly all MPs are on Twitter, and on average tweet 6--8 times a day. \textit{We believe ours is the first work conducting comprehensive quantitative observational studies on elected representatives, specifically covering nearly all sitting MPs in the UK, using Twitter.}



%This paper suggests  MPs use Twitter for both impression management (to tell people of the hard work they are doing, and of their achievements and successes) and for providing a constituency service (informing of surgery hours, helping with citizens' requests etc). 

% \cite{stanyer2008elected} --> MPs have four roles: casework (helping individuals with specific govt problems), projects (helping groups with their efforts), gaining visibility, and party maintenance. Several conflicts arise because of problems with who claims credit and how it is divided, and because MPs doing casework relating to local (rather than central) government may be seen by local councils as stepping on their territory, with MPs often bypassing the local council if it is controlled by opposite party. Territorial heterogeneity (one part of constituency controlled by Labour, another part by Conservative, or one part rich the other poor etc) also plays  a role.

% Models of communication: \ns{we may use this in the MP activities section, esp the bit about symmetric communications}. Most derived from \cite{jackson2004just} which asks the question whether MP interactions are only PR or is it more interactive. Jackson2003 also says that MP communications is mostly asymmetric (\ns{In the $\Rightarrow$ section, we need to test if we find this})
% 1. \textbf{Grunig and Hunt, 1984}. PR as Press agentry model (public communications which may be half truths), public information model (truthful info of use to public), Assymetric and symmetric communications. 
% 2. \textbf{Dozier et al, 1995} Excellence theory of PR. Reconceptualisation of Grunig and Hunt, 
% 3. \textbf{Ferguson 1984}: Relationship management.



% MP efforts to win votes in the offline context has received considerable attention over many years, and our paper benefits from the long scholarship. 

% Following you: Disciplines of listening in social media
% Kate Crawford --> Much social media has been about giving a voice to the citizens. This one says Listening is important for paying attention online. 

% Opinion formation ---> Katz and Lazarsfield. Mass media alone does not change public opinion. Instead it is first sent out by mass media and then gets echoed in a second step by people to their friends. It is in this second social step that opinion is formed.









% The Times commented saying politicians trying to use Twitter appeared to be trying to be cool without being so. Sylvester, R. 2009. Politicians Twitter while the Country Burns. Times Online, 10 March. 

% \pa{Add these-}
% Usage of Twitter for politics elections is new. Studies ranges from taking the case of early sentiments analysis  (https://www.aaai.org/ocs/index.php/ICWSM/ICWSM10/paper/view/1441) to predicting Polls (\url{http://kenbenoit.net/pdfs/Amador_etal_SPP_2017.pdf}) and elections.  
% Moreover, studies are now looking the aspects of ``user following'' behavior and judging the political leaning (Pablo Barbara- Birds from same feather). 
% Emerging as new platform of debate and arguments, social media drives the common audience. Campaigns elections are organized on these platforms and the mechanism is highly studied [http://www.tandfonline.com/doi/abs/10.1080/1369118X.2013.785581] [http://www.tandfonline.com/doi/abs/10.1080/15377857.2014.959686].  Also, winning of Donald Trump in 2016 US election with high usage of social media is widely published[]. 
% Pew Internet suggests that political and civic engagement on social media is among the growing trends. [\url{http://www.pewinternet.org/files/old-media/Files/Reports/2012/PIP_SocialMediaAndPoliticalEngagement_PDF.pdf}]. This is more common in advance democracy where majority of citizens are accessing the technology. Youth engagement is also tracking has been done in UK, USA and Australia. [http://www.tandfonline.com/doi/abs/10.1080/1369118X.2013.871318]
% \ew[]


%
% To the best of our knowledge, we are the first to characterise Facebook Live and to study live social video broadcasts at scale from a user-facing perspective. That said, we identify three core topics of related work.
%
%\vspace{4pt}
%
%\noindent\textbf{Online Video Delivery:} Most prominently, our work overlaps with studies looking at user generated (UGC) video platforms, \eg~\cite{Ameigeiras2012,cha2009analyzing,tyson2013demystifying}. These include user behaviour analysis~\cite{Xing2011} to understand consumption patterns~\cite{Yu2008,Hu2012,Gopalakrishnan2010,Chang2008}. Facebook Live departs from the traditional UGC model of interaction, with users live broadcasting through their mobile device and online social network (rather than simply uploading videos). This allows for a number of new lines of exploration, particularly relating to how \emph{live} videos are created and consumed by social ties. 
%There have been a small number of studies into \emph{live} streaming platforms, including platforms like Akamai~\cite{sripanidkulchai2004analysis}, BBC iPlayer~\cite{nencioni2016score} or CNLive~\cite{li2011measurement}. These professional platforms serve a wide range of international and professional content, although we emphasise that this differs dramatically from the user generated content discussed above. Perhaps the most famous user generated live streaming platform of the day is Twitch, which has seen increasing research attention~\cite{deng2017internet,hamilton2014streaming}. 
%This streams live computer gameplay, but differs from Facebook Live in that it is not mobile, nor integrated within a social network.
%
%
%%%%GT: The below two paragraphs are from the IMC submission. To long for WWW, so merged them into one (above)
%%\noindent\textbf{User Generated Content:} Our work clearly overlaps with traditional studies looking at user generated video platforms, \eg~\cite{Ameigeiras2012,cha2009analyzing,tyson2013demystifying}. Platform characterisation and user behaviour analysis~\cite{Xing2011} is an important part of this work (\eg improvement of content management often needs to be based on the understanding of end users). Most prominently, people have studied the unique properties of users on YouTube~\cite{ding2011broadcast}, and various methods have been developed to help understand this behaviour. For example, mining browsing histories~\cite{Yu2008} and extracting information from online social media~\cite{Hu2012,Gopalakrishnan2010,Chang2008}. Facebook Live departs from this model of interaction, with regular users broadcasting through their mobile device and online social network (rather than simply uploading videos). This allows for a number of new lines of exploration, particularly relating to how live videos are created and consumed by social ties. 
%
%%\noindent\textbf{Live Video Streaming:} Our work is orthogonal to the above, as we explore user behaviour in a related, yet \emph{live} video platform (opposed to these traditional stored content platforms). There have been a small number of studies into live streaming platforms, including platforms like Akamai~\cite{sripanidkulchai2004analysis}, BBC iPlayer~\cite{nencioni2016score} or CNLive~\cite{li2011measurement}. These professional platforms serve a wide range of international and professional content, although we emphasise that this differs dramatically from the user generated content discussed above. Perhaps the most famous user generated live streaming platform of the day is Twitch, which has seen increasing research attention~\cite{deng2017internet,hamilton2014streaming}. Twitch is a platform dedicated to streaming live gameplay, generally through in-game plugins (rather than via a social network). Although this \emph{is} user generated, it is exclusively dedicated to video gameplay. Consequently, it does not cover the mix of professional content and mobile amateur content that Facebook Live offers. It is worth noting that YouTube has also recently introduced a live feature although it has arguably failed to gain the traction of Twitch.
%
%
%
%%We briefly note that Twitch does encompass some social features. Twitch however, centres on a video-centric chat window, rather than integration with social media~\cite{hamilton2014streaming}.
%
%
%\vspace{4pt}
%
%
%\noindent\textbf{Geographical Video Access Patterns:} Another major part of our work is investigating the geographical properties of social broadcast and consumption. There have been a small set of studies looking at the geographical properties of video access. Li \etal~ looked at the the location of viewers watching PPTV in China~\cite{li2014geographic}. They found that a significant portion of videos get at least 70\% of their views from just 3 out of 33 provincial locations. Similar studies have been performed for YouTube, finding that users tend to access videos nearby to them~\cite{brodersen2012youtube}. Whereas studies have been done looking at spatial localities in Facebook~\cite{wittie2010exploiting} and Twitter~\cite{rodrigues2011word}, this has not inspected broadcasts. Interestingly, the integration of live social broadcast with a platform like Facebook also conflates two factors impacting spatial access patterns: \one~Content locality, which is the propensity for content generated nearby to be more relevant to a user; and \two~Social locality, which is the propensity of content generated by friends to be more relevant.  
%
%
%\vspace{4pt}
%
%\noindent\textbf{Social Live Broadcasts:} We take inspiration from the above works, but emphasise \emph{social live broadcasts platforms} such as  Facebook Live and Periscope~\cite{siekkinen2016anatomy,wang2016anatomy} are distinct from these systems in a number of ways. These  allow any user to broadcast themselves (usually from a mobile device) to their friends and possibly other interested parties. Unlike traditional user-generated video platforms, live social streaming drives consumption in realtime. Critically, this is done through direct integration with a social network, notifying online users of the broadcast. 
%This throws up interesting questions that do not emerge in past studies on live platforms. For example, we later explore the social interactions between viewers and broadcasters in realtime. Beyond this, the unique social API of Facebook Live allows us to dive into questions regarding both user locations to understand their impact on content creation and consumption. \looseness=-1
%
%
%To the best of our knowledge, we are the first to study Facebook Live at scale; thus, intentionally, we strive to offer a broad characterisation covering the key novel aspects of the system. There are, however, a small number of studies on related social live streaming platforms. Wang \etal studied Periscope from an infrastructural perspective~\cite{wang2016anatomy}, focussing on understanding how Periscope scales up. This focussed on popular streams, whereas we also focus on the behaviour of unpopular streams (which are more frequently occurring). We also integrate this with exploration of geographical and social properties of the broadcasters. A related paper~\cite{siekkinen2016anatomy} inspected Periscope to capture performance metrics, \eg video quality, stall events, power consumption. Tang \etal focussed on a small set of Meerkat and Periscope broadcasts using crowd sourced analysis and interviews; they focussed on things like motivation for usage~\cite{tang2016meerkat}. This social analysis, however, was based on just 767 (manually analysed) live broadcasts. The focus of our paper is very different. We take a user-facing perspective, empirically exploring the ways users interact with Facebook Live on both a global and regional level. Although, we do this at scale, we also focus on both highly popular and unpopular users to understand system implications for both. 
%
%
%
%
% 


==> sections/reviews.tex <==
\pa{
Item Cards(P as Priority)-
\begin{enumerate}
\item *Done* Add all references to a folder on onedrive or dropbox (also tell what the latest from Lilleker is)
Added references at(\url{https://www.dropbox.com/sh/acewn39y0wrk5l9/AADL_Vb2DbWZdW2mSB43XY8Na?dl=0}) and Lilleker's latest work focuses on - citizen engagements \emph{campaigns, media sharing, EU/Spain elections}.
More references summary in `Added Story's Sec.~\ref{sec:survey}

\item *Done* what fraction botometer accounts were deleted:July Unfollow count (Ans: 93,691 from 12July-13July) and high bot detected in April (17593) and of which (only 379) got deleted in by Aug. Rest high are ok. So 6.2\% follower decreased and 2.11 \%  high bot score mentioner got deleted.

\item How many original tweets are involved in focus windows for each MP. *6787 original tweets in 21,900 focus $\Rightarrow$*.

\item Classify focus points as solicited or unsolicited.

\item Classify the majority source for each MP and what fraction of tweets are from that source. (what fraction of tweets = CDF; Majority source is a bar graph with percentage of MPs with that source as majority). 

\item Remove city of London or greater London from constituency service. [*Updating this now*] Improvements happing when taken post area. UK  121\url{https://upload.wikimedia.org/wikipedia/commons/thumb/f/fe/British_postcode_areas_map.svg/300px-British_postcode_areas_map.svg.png} 

\item MPs self, party and other promotional activity.



\hrule

\item MP Gender verify:  \url{https://researchbriefings.parliament.uk/ResearchBriefing/Summary/CBP-8256} Data (2128 instances) of MPs since 1979. 

\ew{\item MP Staff count average}
\item Constituency service (\#const,email ids:@parliament.uk)
\item Burst time tweets as Proactive/Reactive(did as nonFocus days activity wrt focus days activity). @chhcalling and @PhilipHammondUK falls under reactive as EU controversy and budget decreased their $\Rightarrow$. @patel4witham somewhat proactive as she maintain same level of activity with resigning and congratulations new Minister. 
  
\item Coding Mentioners??
\item Rp Device source for very high focus. 191 MPs have 0.99 (99\%) and higher focus to only one device while doing replies. 121 from which is `Twitter for iPhone` MPs count for Rts and posts for same 0.99 and above focus is 123 and Post 83. \ref{fig:sourceFocus}. Overall, half of the reply focus is $\approx$ 0.9 and post  $\approx$ 0.75 on one device source.   
\end{enumerate}

\ns{New Story Line}

IMP: Report of updates. A table addressing to each review point (sections and page number.)
% Reviews from ICWSM 2018 submission
% \begin{enumerate}
% \item Review 1 (week Reject): Positive about data and looking cross-party interaction. Asking to define less RQs and read more about citizen engagement and re-writing literature survey. Basically, decreasing content from stats and focusing to more on social aspect and insights from activity between the politicians and their constituents. 
% \item Review 2 (week reject): Positive about the engagement pattern and idea of twitter analysis in this space. Suggested that the paper to be more quantitative and lost qualitative aspect of MPs forwarding information from website and engaging in argumentations with citizens.   
% \item Review 3 (week accept): Interested in cross-party and replies behaviors. Attack on popular actors and methods involved.
% \end{enumerate}
% Task Needed and status
% \begin{enumerate}
% \item From R1: Read work by Todd Graham(Leeds), Andres Jungherr (konstanz) and by Darren Lilleker. 
% (Interacting and Representing: can Web 2.0 enhance the roles of an MP?
% BETWEEN BROADCASTING POLITICAL MESSAGES AND INTERACTING WITH VOTERS)
% \item From R2: Add a section of geographic and political details of the users called as citizen. If staff manages Twitter account? Comparision with other politicians and not actors. Address interaction to conclusion. (Add reply thread examples. Add chris bryant backbencher MP example) 
% \item From R3: Check availability, what week of day is more active? is it topic/debate dependent(generalisability)?

% \end{enumerate}
}
